Multi-Objective Path-Based D* Lite

Incremental graph search algorithms such as D* Lite reuse previous, and perhaps partial, searches to expedite subsequent path planning tasks. In this article, we are interested in developing incremental graph search algorithms for path finding problems to simultaneously optimize multiple objectives such as travel risk, arrival time, etc. This is challenging because in a multi-objective setting, the number of "Pareto-optimal" solutions can grow exponentially with respect to the size of the graph. This article presents a new multi-objective incremental search algorithm called Multi-Objective Path-Based D* Lite (MOPBD*) which leverages a path-based expansion strategy to prune dominated solutions. Additionally, we introduce a sub-optimal variant of MOPBD* to improve search efficiency while approximating the Pareto-optimal front. We numerically evaluate the performance of MOPBD* and its variants in various maps with two and three objectives. Results show that our approach is more efficient than search from scratch, and runs up to an order of magnitude faster than the existing incremental method for multi-objective path planning.

==> motivation.tex <==

There are two aspects to be motivated: (1) dynamic environment and (2) multi-objective.
Path planning in dynamic environment has been well motivated by existing work on incremental search~\cite{koenig2005fast,urmson2008autonomous,stentz1995focussed}. In this section, we motivate the consideration of multiple objectives with a toy example and show that why scalarizing multiple objectives into a single-objective is not enough.
As shown in Fig.~\cite{}, the task is to navigate a robot in some uneven terrain, represented as a four-connected grid, from the given start to destination.
The risk score of a cell is equal to the number of obstacles in the proximity, which describes the potential collision risk with the obstacle.
This task minimizes both path length (number of actions of the robot) and accumulated risk along the path.



==> variant.tex <==

\subsection{MOPBD*-i: Fast Computing Non-dominated Subset}\label{sec:variant:mopbd-i}
One of the bottlenecks in MOPBD* is line 8 in Alg.~\ref{alg:edge}, where the $G$-sets of all nodes that are affected are computed. This step requires computing the non-dominated subset $ND(B)$ for a set of vectors $B$.
A naive implementation of $ND(B)$ requires a pairwise comparison between vectors in $B$ and has time complexity $O(|B|^2)$, which can be computationally demanding when the number of nodes affected is large or when $|B|$ is large.

To handle this challenge, we leverage Kung's algorithm~\cite{kung1975finding} within MOPBD* and name the variant as MOPBD*-i (i stands for improvement).
Kung's algorithm is a divide-and-conquer method for fast computation of non-dominated subset for an arbitrary number of objectives and remains the theoretically fastest method till today~\cite{emmerich2018tutorial}.
Kung's algorithm (or ideas similar to it) has been applied in several multi-objective algorithms~\cite{emmerich2018tutorial}.

For presentation purposes, let's focus on the bi-objective setting and we refer the reader to \cite{kung1975finding} for an arbitrary number of objectives.
Given a set of two-dimensional vectors $B$, let's run the following steps to compute $ND(B)$.
\begin{itemize}
	\item Sort the vectors in $B=\{b_k\}$ based on the first component of the vector $b_k(1), \forall b_k \in B$ from small to large, and denote the sorted set of vectors as $B'=\{b'_k\}$.
	\item Introduce an auxiliary scalar value $x_{2,min}$, which is initialized as positive infinity. Initialize the output set $B_{out}$ as an empty set.
	\item Loop over each vector $b'_k \in B'$: If $b'_k(2) > x_{2,min}$, discard $b'_k$; Otherwise, insert $b'_k$ into $B_{out}$ and update $x_{2,min} \gets \min\{x_{2,min}, b'_k(2)\}$.
\end{itemize}
Clearly, the run time complexity of Kung's algorithm in the bi-objective setting is decided by the sorting step, which can be $O(|B|log|B|)$. As shown in Sec.~\ref{sec:results:mopbd-i}, MOPBD*-i can significantly improve the efficiency of MOPBD*.

\subsection{MOPBD*-$\epsilon$: Approximated Pareto-optimal Front}
When there are more than two objectives, computing the exact Pareto-optimal front can be computationally prohibitive due to the enormous size of the Pareto-optimal front.
Correspondingly, how to approximate the Pareto-optimal front efficiently becomes an important problem and several approximation algorithms (such as ~\cite{goldin2021approximate,perny2008near}) have been developed.
In this work, we put no restriction on the number of objectives and we leverage $\epsilon$-dominance~\cite{perny2008near} to enable MOPBD* to approximate the Pareto-optimal front.
%Combining $\epsilon$-dominance with multi-objective search has been investigated and examplified with MOA*~\cite{perny2008near}.

\begin{definition}[$\epsilon$-dominance]
	Given two vectors $a$ and $b$ of length $M$, $a$ $\epsilon$-dominates $b$ (referred as $a \succeq_{\epsilon} b$) if $a(m) \leq (1+\epsilon)\cdot b(m)$ $\forall m \in \{1,2,\dots,M\}$.
\end{definition}
We propose MOPBD*-$\epsilon$ by replacing the dominance comparison in MOPBD* with $\epsilon$-dominance. It's obvious that with a large $\epsilon$, more partial solutions are pruned at each node during the search and the $G$- and $V$-sets at each node have a smaller size. Consequently, the $ND(B)$ operator in line 8 of Alg.~\ref{alg:edge} also runs faster as the input set $B$ becomes smaller, which makes MOPBD* more efficient.

With $\epsilon$-dominance, the sub-optimality accumulates (or say propagates) along the partial solution path~\cite{perny2008near}: the cost vector of the returned path $\pi$ is guaranteed to be $\vec{g}(\pi) \leq (1+\epsilon)^L \cdot \vec{g}(\pi^*)$ for some $\pi^* \in \mathcal{S}^*$, where $L$ is an upper bound on the length of $\pi$, and $\pi^*$ is a Pareto-optimal solution. This property also holds in MOPBD*. 
As a result, MOPBD*-$\epsilon$ is able to trade off between the bounded sub-optimality of the solutions computed and the search efficiency, as shown in Sec.~\ref{sec:results:mopbd_eps}.

